Incorporating Structural Alignment Biases into an Attentional Neural Translation Model

Neural encoder-decoder models of machine translation have achieved impressive results, rivalling traditional translation models. However their modelling formulation is overly simplistic, and omits several key inductive biases built into traditional models. In this paper we extend the attentional neural translation model to include structural biases from word based alignment models, including positional bias, Markov conditioning, fertility and agreement over translation directions. We show improvements over a baseline attentional model and standard phrase-based model over several language pairs, evaluating on difficult languages in a low resource setting.

==> background.tex <==

\section{Encoder-Decoder Models of Translation}

We start by presenting an outline of Sutskever et al.'s \shortcite{sutskever2014sequence} encoder-decoder model,
to introduce our notation and provide the foundations for presenting our extended models.

%\newcommand\vs{\vec{s}}
%\newcommand\vt{\vec{t}}
\newcommand\vE{\vec{e}}

Let $\vs = (s_1, s_2, \ldots, s_I)$, be the input
sentence in the source language (of length $I$), and $\vt = (t_1, t_2, \ldots, t_J)$
be a sentence of length $J$ in the target language. The approach develops a conditional model of the target
given the source, $p(\vt | \vs)$. This is split into two stages:
first encoding, which represents the source as a vector
$\vE$ followed by decoding, $p(\vt; \vE)$, which
proceeds word at a time, in the same manner as a language model.


\paragraph{Encoding}
The encoding step formulates $\vE$  using a recurrent neural
network (RNN), using a recurrence over hidden states,
\begin{align}
\vh_i = \tanh\left( \Wsi \rs_{s_i} +  \Wsh \vh_{i-1} +  \bs \right)
\label{eq:sent-rnn-encoder}
\end{align}
where $\vh_0 \sizev{H}$ is a learned parameter vector, as are
$\Rs \sizem{V_S}{E}$,
$\Wsi \sizem{H}{E}$,  $\Wsh \sizem{H}{H}$ and $\bs \sizev{H}$, with
$H$ the number of hidden units,  $V_S$ the size of the source
vocabulary and $E$ the word embedding
dimensionality.

This forms a `deep' network with a layer for each input
symbol, with each layer combining a symbol with the encoding of all
previous symbols, and with tied weights. The encoding of the final
symbol is then used to represent the input, $\vE = \vh_I$.



\paragraph{Decoding}
The next step is to decode the sequence in the target language, which
is framed as a language model over each symbol, generated left to
right. Again, this is modelled using a RNN, formulated as follows,
\begin{align}
\vg_j = \tanh\left( \Wti \rt_{t_j} +  \Wth \vg_{j-1} +  \bth \right)
\label{eq:sent-rnn-decoder}
\end{align}
where $\vg_0 = \vE$ is the vector encoding of the source, and
$\Rt \sizem{V_T}{E_T}$,
$\Wti \sizem{H}{E_T}$,  $\Wth \sizem{H}{H}$ and $\bth \sizev{H}$, with
 $V_T$ the size of the target
vocabulary.\footnote{We assume the same word embedding and hidden
dimensionality, resp., as for the source, although they could be
different.} At each step $1\le j \le J$ the next target word is
produced,\footnote{$t_1$ is set to a sentinel \texttt{<s>}
  denoting the start of a sequence, and is not generated.}
\begin{align}
t_{j+1} \sim \softmax\left( \Wto \vg_j +  \bto \right)
\end{align}
where $\Wto \sizem{V_T}{H}$ and $\bto \sizev{V_T}$ are parameters.
This process terminates when the sentinel \texttt{</s>} target word is produced,
which forms the final ($J^{th}$) word of the target sequence.

Note that this framework, while conceptually simple, suffers from a
few shortcomings. First, the hidden representation is of fixed length,
and accordingly is unlikely to perform well for arbitrarily long
source sentences. Secondly, the encoding has a bias with respect to
the order of the source sentence, with words at the end contributing
more to the encoding than words at the beginning. A work-around is to
reverse the direction of the source sentence, such that the first
words to be generated in decoding are the last words encoded, however
this is an inadequate solution which becomes clear when considering
the last words to be decoded.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper1_naaclhlt2016"
%%% End: 

